Physically-Plausible Modelling of Biomolecular Systems: A Simplified, Energy-Based Model of the Mitochondrial Electron Transport Chain

Systems biology and whole-cell modelling are demanding increasingly comprehensive mathematical models of cellular biochemistry. These models require the development of simplified models of specific processes which capture essential biophysical features but without unnecessarily complexity. Recently there has been renewed interest in thermodynamically-based modelling of cellular processes. Here we present an approach to developing of simplified yet thermodynamically consistent (hence physically plausible) models which can readily be incorporated into large scale biochemical descriptions but which do not require full mechanistic detail of the underlying processes. We illustrate the approach through development of a simplified, physically plausible model of the mitochondrial electron transport chain and show that the simplified model behaves like the full system.

==> BG-defs.tex <==
%% Referencing and indexing
%%\newcommand{\Index}[1]{\emph{#1}\index{\MakeLowercase{#1}}}
\newcommand{\Index}[1]{\emph{#1}\index{#1}}
\newcommand{\IndeX}[1]{\emph{#1}\index{#1}}
\newcommand{\Ref}[1]{\ref{#1}, p.\pageref{#1}}
\newcommand{\cref}[1]{Chapter~\Ref{#1}}
\newcommand{\aref}[1]{Appendix~\Ref{#1}}
\newcommand{\sref}[1]{\S~\Ref{#1}}
\newcommand{\fref}[1]{Figure~\Ref{#1}}
\newcommand{\eref}[1]{Equation~\eqref{#1}}
\newcommand{\nitem}[3]{\item[#1] #2 \sref{#3}\index{#1}}
\newcommand{\eoe}{$\bm{\Diamond}$} % End of example mark.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "book"
%%% End:


==> BG-figs.tex <==
% Figs
\usepackage{graphicx,subfigure,fancybox,color}
\graphicspath{{./Figs/}}

\newcommand{\Fig}[2]{
 \includegraphics[width=#2\linewidth]{#1.pdf}
}

\newcommand{\RotFig}[2]{
 \includegraphics[width=#2\linewidth,angle=90,origin=c]{#1.pdf}
}

\newcommand{\SubFig}[3]{
 \subfigure[#2]{
   \includegraphics[width=#3\linewidth]{#1.pdf}
   \label{subfig:#1}
 }
}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "book"
%%% End:

